Visualization of High Dynamic Range Solar Imagery and the Radial Histogram Equalizing Filter

Standard visualizations of Extreme Ultraviolet (EUV) solar imagery often fail to convey the full complexity of the Sun's corona, especially in faint off-limb regions. This can leave the misleading impression of the Sun as a bright ball in a dark void, rather than revealing it as the dynamic, structured source of the solar wind and space weather. A variety of enhancement algorithms have been developed to address this challenge, each with its own strengths and tradeoffs. We introduce the Radial Histogram Equalizing Filter (RHEF), a novel hybrid technique that optimizes contrast in high dynamic range solar images. By combining the spatial awareness of radial graded filters with the perceptual benefits of histogram equalization, RHEF reveals faint coronal structures and works out of the box -- without requiring careful parameter tuning or prior dataset characterization. RHEF operates independently on each frame, and it enhances on-disk and off-limb features uniformly across the field of view. For additional control, we also present the Upsilon redistribution function -- a symmetrized cousin of gamma correction -- as an optional post-processing step that provides intuitive programmatic tonal compression. We benchmark RHEF against established methods and offer guidance on filter selection across various applications, with examples from multiple solar instruments provided in an appendix. Implemented and available in both Python sunkit_image and IDL, RHEF enables immediate improvements in solar coronal visualization.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%              MACROS             %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\iin}{I_{in}}
\newcommand{\iio}{I_{out}}


\newtheorem{theorem}{Theorem}
\newcommand{\diff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diffr}[1]{\diff{#1}{r}}
\newcommand{\diffth}[1]{\diff{#1}{\theta}}
\newcommand{\diffz}[1]{\diff{#1}{z}}

\newcommand{\vth}{V_{\theta}}

\newcommand{\twochoices}[2]{\left\{ \begin{array}{lcc}
        \displaystyle #1 \\ \vspace{-10pt} \\
        \displaystyle #2 \end{array} \right. } %}

\newcommand{\threechoices}[3]{\left\{ \begin{array}{lcc}
        #1 \\ #2 \\ #3 \end{array} \right. }    %}

\newcommand{\fourchoices}[4]{\left\{ \begin{array}{lcc}
        #1 \\ #2 \\ #3 \\ #4 \end{array} \right. }      %}

\newcommand{\twovec}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\threevec}[3]{\left(\begin{array}{c} #1 \\ #2 \\ #3 \end{array}\right)}
\newcommand{\twomatrix}[4]{\left(\begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array}\right)}

\newcommand{\linewidthb}{0.8\linewidth} %All the plots are this wide
\newcommand{\enn}{{\bf \hat{n}}}
\newcommand{\appropto}{\mathrel{\vcenter{\offinterlineskip\halign{\hfil$##$\cr\propto\cr\noalign{\kern2pt}\sim\cr\noalign{\kern-2pt}}}}}

% The \ion command
    \newcommand\ion[2]{#1~{%
    \ifx\@currsize\normalsize\small \else
    \ifx\@currsize\small\footnotesize \else
    \ifx\@currsize\footnotesize\scriptsize \else
    \ifx\@currsize\scriptsize\tiny \else
    \ifx\@currsize\large\normalsize \else
    \ifx\@currsize\Large\large
    \fi\fi\fi\fi\fi\fi
    \rmfamily\@Roman{#2}}\relax}% 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%              MACROS             %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \let\hypercontentsline=\contentsline
% \renewcommand{\contentsline}[4]{\hypertarget{toc.#4}{}\hypercontentsline{#1}{#2}{#3}{#4}}
    
% \renewcommand{\em}{\it}



% \IRBprotocol{E927F29.001X}	% optional!
% \ToCisShort	% use this only for 1-page Table of Contents
% \LoFisShort	% use this only for 1-page Table of Figures
% \emptyLoF	% use this if there is no List of Figures
% \LoTisShort	% use this only for 1-page Table of Tables
% \emptyLoT	% use this if there is no List of Tables


%   https://www.colorado.edu/graduateschool/academic-resources/thesis-dissertation-specifications/specifications-preparation-masters-theses#Thesis_Formatting
%   Pages generally are numbered in the upper right hand corner; usual placement is at least 3/4 inch from the top and 1 inch from the right edge.  Centered numbers at the top or bottom of the page are also acceptable.

% Thesis margins should be 1 inch from all edges.
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%       BEGIN DOCUMENT...         %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Definitions for the journal names %%%%%
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apjs}{   {\it Astrophys. J. Sup.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\planss}{ {\it Planetary and Space Sci.}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Affiliations Macros %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\swri}
	{Southwest Research Institute, Boulder, CO}
\newcommand{\ncar}
	{National Center for Atmospheric Research, Boulder, CO}
\newcommand{\predsci}
    {Predictive Science Inc., San Diego, CA}
\newcommand{\umn}
    {University of Minnesota, Minneapolis, MN}
\newcommand{\amu}
    {American University, Washington, DC}
 \newcommand{\msfc}
    {NASA Marshall Space Flight Center, Huntsville, AL}
\newcommand{\cfa}
    {Center for Astrophysics $|$ Harvard \& Smithsonian, Cambridge, MA}
\newcommand{\calb}
    {University of California, Berkeley, CA}
\newcommand{\gsfc}
    {NASA Goddard Space Flight Center, Greenbelt, MD}
\newcommand{\colu}
    {Columbia University, New York, NY}
\newcommand{\adnet}
    {ADNET Systems, Greenbelt, MD}
\newcommand{\jhuapl}
    {Johns Hopkins University Applied Physics Laboratory, Laurel, MD}
\newcommand{\usnrl}
    {U.S. Naval Research Laboratory}
